Reconfiguration of Spanning Trees with Degree Constraint or Diameter Constraint

We investigate the complexity of finding a transformation from a given spanning tree in a graph to another given spanning tree in the same graph via a sequence of edge flips. The exchange property of the matroid bases immediately yields that such a transformation always exists if we have no constraints on spanning trees. In this paper, we wish to find a transformation which passes through only spanning trees satisfying some constraint. Our focus is bounding either the maximum degree or the diameter of spanning trees, and we give the following results. The problem with a lower bound on maximum degree is solvable in polynomial time, while the problem with an upper bound on maximum degree is PSPACE-complete. The problem with a lower bound on diameter is NP-hard, while the problem with an upper bound on diameter is solvable in polynomial time.

==> Spanning Tree Reconfiguration/tikz/cases/basetree.tex <==
\makeatletter
\newcommand*{\getlength}[2]{%
   \pgfmathsetmacro#1{#2}%  Result in `pt`
}
\tikzset{
    partial ellipse/.style args={#1:#2:#3}{insert path={+ (#1:#3) arc (#1:#2:#3)}},
    myvertex/.style = {circle, fill=blue, minimum size=#1, inner sep=0pt, outer sep=0pt},
    myvertex/.default = 6pt, % size of the circle diameter 
    myedge/.style={line width=1.3mm, black!30!green},
    myv/.style={myvertex, fill=red},
    myu/.style={myvertex, fill=red},
    myw/.style={myvertex, fill=red},
    dotted part of curve/.style args={between #1 and #2}{
            postaction={decorate, draw, black,
                    decoration={
                            markings,
                            mark=at position 0 with {\coordinate (u);},
                            mark=between positions 0 and 1 step 6*\pgflinewidth with{\fill[radius=\pgflinewidth*1.5, black] (0,0) circle;},
                            pre=curveto, 
                            pre length=#1*\pgfdecoratedinputsegmentlength,
                            post=moveto, 
                            post length=(1-#2)*\pgfdecoratedinputsegmentlength,
                        }}
    },
    dotted part of curve/.default={between 0.9 and 1},
    get path length/.code={%
    \tikz@addoption{%
      \pgfgetpath\tikz@tmppath%
      \pgfprocessround\tikz@tmppath\tikz@tmppath%
      \pgf@decorate@parsesoftpath\tikz@tmppath\tikz@discard%
      \global\let#1=\pgf@decorate@totalpathlength%
    }%
  }
}
\makeatother

\newcommand{\basetree}{
    \coordinate (c) at (0, 0); 
    \def\cRad{3cm and 2cm} 

    \def\cRone{220} 
    \def\cRtwo{320} 

    \def\cGone{90}
    \def\cGtwo{270} 

    \def\cEone{40} 
    \def\cEtwo{140} 

    \def\EdgeLength{10} 

    \draw (c) [partial ellipse=0:360:\cRad];

    \draw[myedge] (c) [partial ellipse=\cEone - \EdgeLength:\cEone + \EdgeLength:\cRad];
    \node[label={[text=black!30!green,label distance=-5pt]\cEone-180:{$e_1$}}] (e1) at ($(c)+(\cEone:\cRad)$) {};
    \draw[myedge] (c) [partial ellipse=\cEtwo - \EdgeLength:\cEtwo + \EdgeLength:\cRad];
    \node[label={[text=black!30!green,label distance=-5pt]\cEtwo-180:{$e_2$}}] (e2) at ($(c)+(\cEtwo:\cRad)$) {};

    \node[label={[label distance=-8pt]\cEone:{$q_1$}}] at (e1) {\Large $\times$}; 
    \node[label={[label distance=-8pt]\cEtwo:{$q_2$}}] at (e2) {\Large $\times$}; 

    \node[myvertex, label=\cRone:{$r_1$}] (r1) at ($(c)+(\cRone:\cRad)$) {};
    \node[myvertex, label=\cRtwo:{$r_2$}] (r2) at ($(c)+(\cRtwo:\cRad)$) {};
    \node[myvertex, label=\cGone:{$g_1$}] (g1) at ($(c)+(\cGone:\cRad)$) {};
    \node[myvertex, label=\cGtwo:{$g_2$}] (g2) at ($(c)+(\cGtwo:\cRad)$) {};
}

==> tikz/cases/basetree.tex <==
\makeatletter
\newcommand*{\getlength}[2]{%
   \pgfmathsetmacro#1{#2}%  Result in `pt`
}
\tikzset{
    partial ellipse/.style args={#1:#2:#3}{insert path={+ (#1:#3) arc (#1:#2:#3)}},
    myvertex/.style = {circle, fill=blue, minimum size=#1, inner sep=0pt, outer sep=0pt},
    myvertex/.default = 6pt, % size of the circle diameter 
    myedge/.style={line width=1.3mm, black!30!green},
    myv/.style={myvertex, fill=red},
    myu/.style={myvertex, fill=red},
    myw/.style={myvertex, fill=red},
    dotted part of curve/.style args={between #1 and #2}{
            postaction={decorate, draw, black,
                    decoration={
                            markings,
                            mark=at position 0 with {\coordinate (u);},
                            mark=between positions 0 and 1 step 6*\pgflinewidth with{\fill[radius=\pgflinewidth*1.5, black] (0,0) circle;},
                            pre=curveto, 
                            pre length=#1*\pgfdecoratedinputsegmentlength,
                            post=moveto, 
                            post length=(1-#2)*\pgfdecoratedinputsegmentlength,
                        }}
    },
    dotted part of curve/.default={between 0.9 and 1},
    get path length/.code={%
    \tikz@addoption{%
      \pgfgetpath\tikz@tmppath%
      \pgfprocessround\tikz@tmppath\tikz@tmppath%
      \pgf@decorate@parsesoftpath\tikz@tmppath\tikz@discard%
      \global\let#1=\pgf@decorate@totalpathlength%
    }%
  }
}
\makeatother

\newcommand{\basetree}{
    \coordinate (c) at (0, 0); 
    \def\cRad{3cm and 2cm} 

    \def\cRone{220} 
    \def\cRtwo{320} 

    \def\cGone{90}
    \def\cGtwo{270} 

    \def\cEone{40} 
    \def\cEtwo{140} 

    \def\EdgeLength{10} 

    \draw (c) [partial ellipse=0:360:\cRad];

    \draw[myedge] (c) [partial ellipse=\cEone - \EdgeLength:\cEone + \EdgeLength:\cRad];
    \node[label={[text=black!30!green,label distance=-5pt]\cEone-180:{$e_1$}}] (e1) at ($(c)+(\cEone:\cRad)$) {};
    \draw[myedge] (c) [partial ellipse=\cEtwo - \EdgeLength:\cEtwo + \EdgeLength:\cRad];
    \node[label={[text=black!30!green,label distance=-5pt]\cEtwo-180:{$e_2$}}] (e2) at ($(c)+(\cEtwo:\cRad)$) {};

    \node[label={[label distance=-8pt]\cEone:{$q_1$}}] at (e1) {\Large $\times$}; 
    \node[label={[label distance=-8pt]\cEtwo:{$q_2$}}] at (e2) {\Large $\times$}; 

    \node[myvertex, label=\cRone:{$r_1$}] (r1) at ($(c)+(\cRone:\cRad)$) {};
    \node[myvertex, label=\cRtwo:{$r_2$}] (r2) at ($(c)+(\cRtwo:\cRad)$) {};
    \node[myvertex, label=\cGone:{$g_1$}] (g1) at ($(c)+(\cGone:\cRad)$) {};
    \node[myvertex, label=\cGtwo:{$g_2$}] (g2) at ($(c)+(\cGtwo:\cRad)$) {};
}
